WaveMo: Learning Wavefront Modulations to See Through Scattering

Imaging through scattering media is a fundamental and pervasive challenge in fields ranging from medical diagnostics to astronomy. A promising strategy to overcome this challenge is wavefront modulation, which induces measurement diversity during image acquisition. Despite its importance, designing optimal wavefront modulations to image through scattering remains under-explored. This paper introduces a novel learning-based framework to address the gap. Our approach jointly optimizes wavefront modulations and a computationally lightweight feedforward "proxy" reconstruction network. This network is trained to recover scenes obscured by scattering, using measurements that are modified by these modulations. The learned modulations produced by our framework generalize effectively to unseen scattering scenarios and exhibit remarkable versatility. During deployment, the learned modulations can be decoupled from the proxy network to augment other more computationally expensive restoration algorithms. Through extensive experiments, we demonstrate our approach significantly advances the state of the art in imaging through scattering media. Our project webpage is at https://wavemo-2024.github.io/.

==> backup/1_intro_brandon.tex <==
\section{Introduction}
\label{sec:intro}
%Scattering and related optical aberrations are ubiquitous in imaging and can be caused by a broad range of factors including fog, raindrops, murky water, atmospheric turbulence, fiber bundles, and human skin and tissue~\cite{gigan2022roadmap,yoon2020deep,watnik2018wavefront}. When light passes through such media, its phase is irregularly delayed and
%its ``wavefront'' becomes distorted. These distortions blur and warp any images captured through
%the scatterer. Solving the imaging-through-scattering problem would have profound implications in autonomous navigation, microscopy, endoscopy, astronomy, remote sensing, and other applications.
Imaging through scattering media presents a significant challenge across diverse scenarios, ranging from navigating with fog, rain, or murky water to recovering intricate structures through human skin and tissue~\cite{gigan2022roadmap,yoon2020deep,watnik2018wavefront}. The core of this challenge are the phase delays of light as it goes through these media, resulting in wavefront distortions that manifest as blurred or distorted images. Effectively addressing this issue is crucial not only for improving image clarity but also for unlocking new possibilities in various fields, such as autonomous navigation, medical imaging, and astronomy.

Wavefront passing through scattering media is disrupted, often leading to a significant loss of information in the observed image.
From the frequency domain perspective, 
%From the frequency domain perspective, the scattering media can significantly disrupt the frequency components of a target scene, either by destructively interfering with them or by scattering them outside the imaging sensor.
frequencies that are already lost during acquisition are difficult to recover using computational methods.
Existing methods predominantly rely on prior information about the target scene, such as the hand-crafted total variation and Tikhonov regularizations, or data-driven methods using trained neural networks.
These methods do not fundamentally resolve the inherent ill-posedness of this challenge, as they essentially speculates on the missing frequencies based on those that have been preserved.
The question naturally arises: Can we prevent the loss of information during acquisition? 

A promising solution is to actively modulate the scattered wavefront during acquisition, in hopes that applying multiple modulations increases the chance that a frequency component is preserved.
This approach is related to phase diversity imaging~\cite{gonsalves1982phase,paxman1992joint,vogel1998fast,thelen1999maximum,kner2013phase,xin2019object,kang2023coordinate,reiser2023phase}, which typically captures multiple scattered images of a static scene with different modulations applied using deformable mirrors or spatial light modulators (SLM).
However, phase diversity imaging traditionally was limited to imaging simple scenes with mild optical aberrations, and the phase modulations were often selected based on simple heuristics.
The recent development of neural wavefront shaping (NeuWS)~\cite{feng2023neuws} brings a significant breakthrough by leveraging recent innovations in machine learning and enables imaging high-resolution and dynamic scenes through severe aberrations.
Still, the wavefront modulations applied by NeuWS during acquisition were chosen randomly without much consideration over their impact on frequency preservation.

%Wavefront shaping lets you image through scattering
%In principle,  one can use SLMs to ``shape'' the wavefront of incoming light and undo scattering-induced distortions~\cite{booth2014adaptive,hampson2021adaptive,vellekoop2007focusing,mosk2012controlling,yeminy2021guidestar}. This technique to imaging through scattering is known as wavefront shaping (WS) and is arguably the most effective approach to date.


\begin{figure}[t]
  \centering
   \includegraphics[width=\linewidth]{sec/figs/teaser.pdf}
   \caption{\textbf{Learned Wavefront Modulations}. During image acquisition, we shape the wavefront of scattered light with a series of learned modulation patterns and capture a set of image measurements. 
   %We can then solve a maximum-likelihood estimation problem (or employ a feedforward neural network) to recover the obstructed scene. 
   We can then recover the scene behind the scattering medium by feeding the modulated measurements to supervised or unsupervised reconstruction methods.
   Using a state-of-the-art unsupervised method~\cite{feng2023neuws}, our learned modulations drastically improve the reconstruction quality compared to the previous approach~\cite{feng2023neuws} that applies random modulations during acquisition.}
   \label{fig:onecol}
\end{figure}

%Most approaches to wavefront shaping require guidestars
%However, the majority of WS techniques---and imaging-through-scattering techniques generally---require one to perform wavefront sensing; in order to correct a wavefront error, one must measure it. Unfortunately, measuring a wavefront typically requires controlled illumination, point-by-point scanning, static scenes, and, most significantly, the presence of a few bright points in the scene being images, i.e., ``guidestars''~\cite{vellekoop2012digital,horstmeyer2015guidestar,aizik2022fluorescent,lai2015photoacoustically,xu2011time,hsieh2010digital,papadopoulos2017scattering}.  The guidestar requirement has placed severely restrict where and when WS can be performed. 

%Phase diversity is a powerful guidestar-free approach to imaging through aberrations
%PDI is a powerful {\em guidestar-free} approach to imaging through optical aberrations. 
%PDI methods captures a sequence of measurements where each measurement introduces an additional {known} wavefront error---typically just defocus---into the measurement~\cite{gonsalves1982phase,paxman1992joint,vogel1998fast,thelen1999maximum,kner2013phase,xin2019object,kang2023coordinate,reiser2023phase}. Much like the coded diffraction patterns employed in the context of phase retrieval~\cite{candes2015phaseCDP}, this modulation process adds diversity to the measurements and makes the obstructed scene easier to reconstruct. 


%NeuWS extends phase diverstiy imaging to image through severe optical aberrations
%Until recently, PDI approaches were restricted to imaging simple scenes through the relatively mild (smooth and regular) optical aberrations.
%However, a breakthrough neural wavefront shaping (NeuWS) PDI technique was recently developed that combines high-resolution SLM based modulation with recent developments in machine learning (implicit neural representations~\cite{sitzmann2020implicit}) to image high-resolution, non-sparse static and dynamic scenes through severe optical aberrations~\cite{feng2023neuws}.
%NeuWS represents the state-of-the-art in guidestar-free imaging through scattering.

%Neural wavefront shaping is a breakthrough phase diversity imaging approach capable imaging through severe optical aberrations.


%Phase diversity imaging and NeuWS rely upon slow iterative algorithms and simple heuristics.


% Imaging through scattering is challenging because in general a scattering media's phase errors are unknown. 
% \textcolor{red}{Unknown and ill-posed are distinct problems. You could perfectly know the scattering media, but its forward model may not be invertible.}
% As a result, the inverse problems associated with imaging through scattering are often very ill-posed. 
% Imaging through scattering is challenging because the scattering process is lossy. 
% From the frequency domain perspective, the scattering media destroys some of the target scene's frequencies, either by destructively interfering with them or by scattering them outside the imaging sensor. If those frequencies are not captured in the measurement, it becomes difficult to faithfully recover them.

% %Imaging through scattering is hard
% Imaging through scattering is challenging because, in general, the scattering process is {\em unknown} and {\em lossy}. In the context of imaging an incoherent scene through an isoplanatic (spatially invariant) aberration, imaging through scattering can be framed as a blind deconvolution problem. In general, to image through scattering one must both recover the scattering-induced blur kernel and then invert (optically or computational) the scattering process to recover missing frequency content in the image.

%the noisy and corrupted measurements $I$ are related to the object of interest $O$ through 
% \begin{align}
%     I=O*H+Z,
% \end{align}
% where $H$ denotes an unknown blur kernel and $Z$ denotes denotes.




% %How existing methods deal with the imaging through scattering problem
% Many techniques have been developed to image through scattering media. If can can create a contre

% To recover the missing signal frequencies due to scattering media, most existing methods rely on prior information of the target scene, either hand-crafted or data-driven. Hand-crafted priors include but are not limited to total variation and Tikhonov regularization. Alternatively, data-driven priors require training a neural network to learn the mapping between distorted measurements and clean target scenes. A trained neural network can be either directly used to predict an estimate of the target in a feed-forward manner, or integrated into iterative optimization frameworks. 

% roughly fall into two categories: (1) data-driven supervised learning approaches and (2) unsupervised iterative optimization approaches. However, both categories suffer from said ill-posedness issue. As a result, data-driven feed-forward approaches tend to hallucinate realistic yet fake features in their reconstruction, while unsupervised approaches might lead to undesired artifacts, and tend to be much slower than feed-forward approaches.  Efforts have been made to fuse the two categories by using a data-driven neural network as a regularizer for iterative optimization approaches, 
 
% Although the aforementioned priors can help fill in the missing frequencies, they do not fundamentally escape the ill-posed nature of this problem --- they merely circumvent it by ``guessing'' or ``hallucinating'' the missing frequencies based on the preserved ones. The more frequencies are destroyed by the scattering media, the more inaccurate and error prone these reconstructions become. 
% Phase diversity imaging provides a mechanism to prevent these frequencies from being destroyed in the first place.
% %But can we prevent these frequencies from being destroyed in the first place? Yes, through phase diversity imaging. 

%\textcolor{red}{Need to rework this transition. PDI has been around for 30 years.}
%Recently, phase diversity imaging has emerged as a promising tool for imaging through scattering media, thanks to the development of deformable mirror arrays and spatial light modulators (SLM). These devices are able to arbitrarily shape the wavefront of incoming light by displaying phase modulation patterns in real-time (up to 1,000 fps). 
%\subsection{Phase Diversity Imaging}


%Phase diversity imaging, \textcolor{red}{illustrated in Figure XXX}, works by capturing a sequence of measurements -- each time the camera captures one measurement through the scattering media with a different phase modulation pattern. Its key idea is that a single phase modulation can make some of the frequencies better preserved, and make others worse preserved; but by applying multiple phase modulations in sequence, every frequency gets better preserved by at least one of the phase modulations; thus by leveraging all measurements, it can reduce ill-posedness. Recent works have demonstrated the advantage of phase diversity imaging via unsupervised iterative optimization approaches, of which the used phase modulation sequences are chosen by simple heuristics.



% Recent works have demonstrated the superior advantage of phase diversity imaging by using generic algorithms and neural representation, both of which are done in an unsupervised and iterative manner. 

% It should also be noted that this "multiple phase modulation" ability makes this line of work fundamentally different from the usage of single phase mask, as single phase mask would not be able to 


% It should be noted that this "multiple phase modulation" ability makes phase diversity imaging fundementally different from. 

% This differs from single phase mask that xxx.In comparison to using a single phase mask, 
% talk about single phase mask.

In this paper, we take a significant step towards a more systematic and principled approach in designing effective modulations that induces phase diversity during image acquisition. 
Moving beyond the traditional reliance on simple heuristics for determining modulation patterns, our method combines the strengths of differentiable optimization and data-driven learning.
Central to our approach is the novel integration of the optical model of wavefront modulations with a {\it proxy} reconstruction network, resulting in a fully differentiable system.
This integration allows for the simultaneous optimization of both the proxy reconstruction network and the modulation patterns, which are optimized end-to-end based on a large, simulated training dataset.
While imaging through scattering often requires iterative optimization algorithms because deep-learned feedforward networks often fail to generalize outside their training domain, this paper presents an intriguing twist by showing that, the training of a {\it hard-to-generalize} network can actually become a useful proxy for us to learn {\it generalizable} modulations.
Crucially, this proxy feedforward network allows us to bypass the expensive backpropagation computation through an iterative reconstruction algorithm, which would be necessary, but hopelessly impractical, if we were to naively optimize the modulations: each optimization step would require us to finish an entire iterative reconstruction algorithm.
As will be shown, our learned modulations significantly enhance the reconstruction capability of both our deep-learned feedforward proxy network and a state-of-the-art iterative optimization-based method for imaging through scattering.
%Our framework is distinct in its ability to integrate data-driven insights about the scattering impact on wavefront into the design of wavefront modulations.
%Furthermore, the versatility of our framework is highlighted by its dual functionality: while our trained network exhibits strong generalization capabilities on unseen test data captured with our learned modulations, the modulations can also be effortlessly incorporated into existing imaging methods that employ iterative optimization.

%\subsection{Our Contribution}

% \textcolor{red}{I don't like this paragraph's narrative. This reads as improving how priors are incorporated. I'd prefer to talk about introducing a principled and powerful way to select modulation patterns.}
% With the knowledge of phase diversity imaging in mind, let us rethink the strategy of incorporating prior knowledge. While the research community has spent a ton of efforts on imposing priors in the image space to improve the image reconstruction quality,  we explore a new research direction: \textit{can we impose prior information on the design of phase-modulation-sequence such that the resulted phase diversity imaging system can preserve more frequencies?} It should be noted that the latter direction is complementary to the former -- if more frequencies get preserved, then subsequently, the problem would become much less ill-posed, and the priors on image space would also work better. 

%This paper develops a powerful learning-based approach for designing and optimizing PDI modulation patterns and reconstruction algorithms. 
%Our approach integrates differentiable optical models with feedforward image reconstruction algorithms to form a fully differentiable model of our imaging system that we can optimize end-to-end with training data and back-propagation. 

%optimize a learning-based PDI system end-to-end

%designing and optimizing learning-based phase diversity imaging systems.

%Contrary to the heuristically chosen phase modulation sequences used in previous phase diversity imaging approaches, in this work, we propose to use end-to-end learning to embed prior information of scattering media into our phase modulation sequence design. With a differentiable model for scattering media, our phase modulation sequence is jointly optimized with a feed-forward reconstruction neural network.  

The contributions of this paper include:
\begin{itemize}[leftmargin=.3in]
  \item We present a novel end-to-end learning framework to optimize wavefront modulations during acquisition to enhance our abilities to see through scattering.
  \item We demonstrate in both simulated and physical experiments that our learned modulations substantially improve image reconstruction quality and effectively generalize to unseen targets and scattering media.
  \item We show that the learned modulations can be decoupled from the jointly trained reconstruction network and significantly enhance the reconstruction quality of state-of-the-art unsupervised approaches.
  \end{itemize}

% We hope that our work can inspire the research community to to

% More specifically, we make the following contributions:. In this work, we investigate the optimal design of phase modulation sequence, in hope of preserving the most amount of frequency information against scattering media. 

% However, one limitation of previous wavefront modulation methods is that they use randomly generated modulation patterns. It has not yet been investigated whether using randomly generated phase modulation patterns leads to sub-optimal performance. In this paper, we make the following contributions:

% a new research direction. We hope that our work can inspire the research community to 

% ts key idea being improving the conditioning of the imaging system. More specifically, 
    

% \subsection{Contributions}




==> backup/1_intro_brandon_no_comments.tex <==
\section{Introduction}
\label{sec:intro}
Imaging through scattering media presents a significant challenge across diverse scenarios, ranging from navigating with fog, rain, or murky water to recovering intricate structures through human skin and tissue~\cite{gigan2022roadmap,yoon2020deep,watnik2018wavefront}. The core of this challenge are the phase delays of light as it goes through these media, resulting in wavefront distortions that manifest as blurred or distorted images. Effectively addressing this issue is crucial not only for improving image clarity but also for unlocking new possibilities in various fields, such as autonomous navigation, medical imaging, and astronomy.

Wavefront passing through scattering media is disrupted, often leading to a significant loss of information in the observed image.
From the frequency domain perspective, 
%From the frequency domain perspective, the scattering media can significantly disrupt the frequency components of a target scene, either by destructively interfering with them or by scattering them outside the imaging sensor.
frequencies that are already lost during acquisition are difficult to recover using computational methods.
Existing methods predominantly rely on prior information about the target scene, such as the hand-crafted total variation and Tikhonov regularizations, or data-driven methods using trained neural networks.
These methods do not fundamentally resolve the inherent ill-posedness of this challenge, as they essentially speculates on the missing frequencies based on those that have been preserved.
The question naturally arises: Can we prevent the loss of information during acquisition? 

A promising solution is to actively modulate the scattered wavefront during acquisition, in hopes that applying multiple modulations increases the chance that a frequency component is preserved.
This approach is related to phase diversity imaging~\cite{gonsalves1982phase,paxman1992joint,vogel1998fast,thelen1999maximum,kner2013phase,xin2019object,kang2023coordinate,reiser2023phase}, which typically captures multiple scattered images of a static scene with different modulations applied using deformable mirrors or spatial light modulators (SLM).
However, phase diversity imaging traditionally was limited to imaging simple scenes with mild optical aberrations, and the phase modulations were often selected based on simple heuristics.
The recent development of neural wavefront shaping (NeuWS)~\cite{feng2023neuws} brings a significant breakthrough by leveraging recent innovations in machine learning and enables imaging high-resolution and dynamic scenes through severe aberrations.
Still, the wavefront modulations applied by NeuWS during acquisition were chosen randomly without much consideration over their impact on frequency preservation.

%Wavefront shaping lets you image through scattering
%In principle,  one can use SLMs to ``shape'' the wavefront of incoming light and undo scattering-induced distortions~\cite{booth2014adaptive,hampson2021adaptive,vellekoop2007focusing,mosk2012controlling,yeminy2021guidestar}. This technique to imaging through scattering is known as wavefront shaping (WS) and is arguably the most effective approach to date.


\begin{figure}[t]
  \centering
   \includegraphics[width=\linewidth]{sec/figs/teaser.pdf}
   \caption{\textbf{Learned Wavefront Modulations}. During image acquisition, we shape the wavefront of scattered light with a series of learned modulation patterns and capture a set of image measurements. 
   %We can then solve a maximum-likelihood estimation problem (or employ a feedforward neural network) to recover the obstructed scene. 
   We can then recover the scene behind the scattering medium by feeding the modulated measurements to supervised or unsupervised reconstruction methods.
   Using a state-of-the-art unsupervised method~\cite{feng2023neuws}, our learned modulations drastically improve the reconstruction quality compared to the previous approach~\cite{feng2023neuws} that applies random modulations during acquisition.}
   \label{fig:onecol}
\end{figure}


In this paper, we take a significant step towards a more systematic and principled approach in designing effective modulations that induces phase diversity during image acquisition. 
Moving beyond the traditional reliance on simple heuristics for determining modulation patterns, our method combines the strengths of differentiable optimization and data-driven learning.
Central to our approach is the novel integration of the optical model of wavefront modulations with a {\it proxy} reconstruction network, resulting in a fully differentiable system.
This integration allows for the simultaneous optimization of both the proxy reconstruction network and the modulation patterns, which are optimized end-to-end based on a large, simulated training dataset.
While imaging through scattering often requires iterative optimization algorithms because deep-learned feedforward networks often fail to generalize outside their training domain, this paper presents an intriguing twist by showing that, the training of a {\it hard-to-generalize} network can actually become a useful proxy for us to learn {\it generalizable} modulations.
Crucially, this proxy feedforward network allows us to bypass the expensive backpropagation computation through an iterative reconstruction algorithm, which would be necessary, but hopelessly impractical, if we were to naively optimize the modulations: each optimization step would require us to finish an entire iterative reconstruction algorithm.
As will be shown, our learned modulations significantly enhance the reconstruction capability of both our deep-learned feedforward proxy network and a state-of-the-art iterative optimization-based method for imaging through scattering.

The contributions of this paper include:
\begin{itemize}[leftmargin=.3in]
  \item We present a novel end-to-end learning framework to optimize wavefront modulations during acquisition to enhance our abilities to see through scattering.
  \item We demonstrate in both simulated and physical experiments that our learned modulations substantially improve image reconstruction quality and effectively generalize to unseen targets and scattering media.
  \item We show that the learned modulations can be decoupled from the jointly trained reconstruction network and significantly enhance the reconstruction quality of state-of-the-art unsupervised approaches.
  \end{itemize}

==> backup/1_intro_chris.tex <==
\section{Introduction}
\label{sec:intro}
Scattering and related optical aberrations are ubiquitous in imaging and can be caused by a broad range of factors including fog, raindrops, murky water, atmospheric turbulence, fiber bundles, and human skin and tissue~\cite{gigan2022roadmap,yoon2020deep,watnik2018wavefront}. When light passes through such media, its phase is irregularly delayed and
its ``wavefront'' becomes distorted. These distortions blur and warp any images captured through
the scatterer. Solving the imaging-through-scattering problem would have profound implications in autonomous navigation, microscopy, endoscopy, astronomy, remote sensing, and other applications.

\begin{figure}[t]
  \centering
   \includegraphics[width=\linewidth]{sec/figs/teaser.pdf}
   \caption{\textbf{Learned Wavefront Modulations}. During image acquisition, we shape the wavefront of scattered light with a series of learned modulation patterns and capture a set of image measurements. 
   %We can then solve a maximum-likelihood estimation problem (or employ a feedforward neural network) to recover the obstructed scene. 
   We can then recover the scene behind the scattering medium by feeding the modulated measurements to supervised or unsupervised reconstruction methods.
   Using a state-of-the-art unsupervised method~\cite{feng2023neuws}, our learned modulations drastically improve the reconstruction quality compared to the previous approach~\cite{feng2023neuws} that applies random modulations during acquisition.}
   \label{fig:onecol}
\end{figure}

From the frequency domain perspective, the effect of an (incoherently illuminated) scene passing through scattering is the destruction/filtering of frequency content. 
Recovering these lost frequencies is very difficult using purely computational methods. %A question naturally arises: Can we modify the measurement process to prevent the loss of information during acquisition? 
Wavefront modulation and phase diversity imaging are powerful approaches to image through optical aberrations which modify the measurement process to preserve and recover frequency content.  
These methods captures a sequence of measurements where each measurement introduces an additional {known} wavefront error---typically just defocus---into the measurement~\cite{gonsalves1982phase,paxman1992joint,vogel1998fast,thelen1999maximum,kner2013phase,xin2019object,kang2023coordinate,reiser2023phase}. Much like the coded diffraction patterns employed in the context of phase retrieval~\cite{candes2015phaseCDP}, this modulation process adds diversity to the measurements and makes the obstructed scene easier to reconstruct. 

Until recently, such approaches were restricted to imaging simple scenes through the relatively mild (smooth and regular) optical aberrations.
However, a breakthrough neural wavefront shaping (NeuWS) technique was recently developed that combines high-resolution SLM based modulation with recent developments in machine learning (implicit neural representations~\cite{sitzmann2020implicit}) to image high-resolution, non-sparse static and dynamic scenes through severe optical aberrations~\cite{feng2023neuws}.
NeuWS represents the state-of-the-art in guidestar-free imaging through scattering.

\subsection{Our Contribution}

This paper develops a powerful learning-based approach for designing and optimizing wavefront modulation patterns. 
Our approach integrates differentiable optical models with feedforward {\em proxy} image reconstruction algorithms to form a fully differentiable model of our imaging system that we can optimize end-to-end with training data and back-propagation. 

While imaging through scattering often requires iterative optimization algorithms because deep-learned feedforward networks often fail to generalize outside their training domain, this paper demonstrates the remarkable finding that training a {\it hard-to-generalize} network can become a useful proxy allowing us to learn {\it generalizable} modulations.
Crucially, this proxy feedforward network allows us to bypass the expensive backpropagation computation through an iterative reconstruction algorithm, which would be necessary, but hopelessly impractical, if we were to naively optimize the modulations: each optimization step would require us to finish an entire iterative reconstruction algorithm.
As will be shown in our extensive experiments on both simulated and real-world data, our learned modulations significantly enhance the reconstruction capability of both our deep-learned feedforward proxy network and a state-of-the-art iterative optimization-based method for imaging through scattering.

The contributions of this paper include:
\begin{itemize}[leftmargin=.3in]
  \item We present a novel end-to-end learning framework to optimize wavefront modulations during acquisition to enhance our abilities to see through scattering.
  \item We demonstrate in both simulated and physical experiments that our learned modulations substantially improve image reconstruction quality and effectively generalize to unseen targets and scattering media.
  \item We show that the learned modulations can be decoupled from the jointly-trained proxy reconstruction network and significantly enhance the reconstruction quality of state-of-the-art unsupervised approaches.
  \end{itemize}

\iffalse

%Scattering and related optical aberrations are ubiquitous in imaging and can be caused by a broad range of factors including fog, raindrops, murky water, atmospheric turbulence, fiber bundles, and human skin and tissue~\cite{gigan2022roadmap,yoon2020deep,watnik2018wavefront}. When light passes through such media, its phase is irregularly delayed and
%its ``wavefront'' becomes distorted. These distortions blur and warp any images captured through
%the scatterer. Solving the imaging-through-scattering problem would have profound implications in autonomous navigation, microscopy, endoscopy, astronomy, remote sensing, and other applications.
Imaging through scattering media presents a significant challenge across diverse scenarios, ranging from navigating with fog, rain, or murky water to recovering intricate structures through human skin and tissue~\cite{gigan2022roadmap,yoon2020deep,watnik2018wavefront}. The core of this challenge are the phase delays of light as it goes through these media, resulting in wavefront distortions that manifest as blurred or distorted images. Effectively addressing this issue is crucial not only for improving image clarity but also for unlocking new possibilities in various fields, such as autonomous navigation, medical imaging, and astronomy.

Wavefront passing through scattering media is disrupted, often leading to a significant loss of information in the observed image.
From the frequency domain perspective, 
%From the frequency domain perspective, the scattering media can significantly disrupt the frequency components of a target scene, either by destructively interfering with them or by scattering them outside the imaging sensor.
frequencies that are already lost during acquisition are difficult to recover using computational methods.
Existing methods predominantly rely on prior information about the target scene, such as the hand-crafted total variation and Tikhonov regularizations, or data-driven methods using trained neural networks.
These methods do not fundamentally resolve the inherent under-determinedness of this challenge, as they essentially speculates on the missing frequencies based on those that have been preserved.
The question naturally arises: Can we prevent the loss of information during acquisition? 

A promising solution is to actively modulate the scattered wavefront during acquisition, in hopes that applying multiple modulations increases the chance that a frequency component is preserved.
This approach is related to phase diversity imaging~\cite{gonsalves1982phase,paxman1992joint,vogel1998fast,thelen1999maximum,kner2013phase,xin2019object,kang2023coordinate,reiser2023phase}, which typically captures multiple scattered images of a static scene with different modulations applied using deformable mirrors or spatial light modulators (SLM).
However, phase diversity imaging traditionally was limited to imaging simple scenes with mild optical aberrations, and the phase modulations were often selected based on simple heuristics.
The recent development of neural wavefront shaping (NeuWS)~\cite{feng2023neuws} brings a significant breakthrough by leveraging recent innovations in machine learning and enables imaging high-resolution and dynamic scenes through severe aberrations.
Still, the wavefront modulations applied by NeuWS during acquisition were chosen randomly without much consideration over their impact on frequency preservation.

%Wavefront shaping lets you image through scattering
%In principle,  one can use SLMs to ``shape'' the wavefront of incoming light and undo scattering-induced distortions~\cite{booth2014adaptive,hampson2021adaptive,vellekoop2007focusing,mosk2012controlling,yeminy2021guidestar}. This technique to imaging through scattering is known as wavefront shaping (WS) and is arguably the most effective approach to date.


\begin{figure}[t]
  \centering
   \includegraphics[width=\linewidth]{sec/figs/teaser.pdf}
   \caption{\textbf{Learned Wavefront Modulations}. During image acquisition, we shape the wavefront of scattered light with a series of learned modulation patterns and capture a set of image measurements. 
   %We can then solve a maximum-likelihood estimation problem (or employ a feedforward neural network) to recover the obstructed scene. 
   We can then recover the scene behind the scattering medium by feeding the modulated measurements to supervised or unsupervised reconstruction methods.
   Using a state-of-the-art unsupervised method~\cite{feng2023neuws}, our learned modulations drastically improve the reconstruction quality compared to the previous approach~\cite{feng2023neuws} that applies random modulations during acquisition.}
   \label{fig:onecol}
\end{figure}

%Most approaches to wavefront shaping require guidestars
%However, the majority of WS techniques---and imaging-through-scattering techniques generally---require one to perform wavefront sensing; in order to correct a wavefront error, one must measure it. Unfortunately, measuring a wavefront typically requires controlled illumination, point-by-point scanning, static scenes, and, most significantly, the presence of a few bright points in the scene being images, i.e., ``guidestars''~\cite{vellekoop2012digital,horstmeyer2015guidestar,aizik2022fluorescent,lai2015photoacoustically,xu2011time,hsieh2010digital,papadopoulos2017scattering}.  The guidestar requirement has placed severely restrict where and when WS can be performed. 

%Phase diversity is a powerful guidestar-free approach to imaging through aberrations
%PDI is a powerful {\em guidestar-free} approach to imaging through optical aberrations. 
%PDI methods captures a sequence of measurements where each measurement introduces an additional {known} wavefront error---typically just defocus---into the measurement~\cite{gonsalves1982phase,paxman1992joint,vogel1998fast,thelen1999maximum,kner2013phase,xin2019object,kang2023coordinate,reiser2023phase}. Much like the coded diffraction patterns employed in the context of phase retrieval~\cite{candes2015phaseCDP}, this modulation process adds diversity to the measurements and makes the obstructed scene easier to reconstruct. 


%NeuWS extends phase diverstiy imaging to image through severe optical aberrations
%Until recently, PDI approaches were restricted to imaging simple scenes through the relatively mild (smooth and regular) optical aberrations.
%However, a breakthrough neural wavefront shaping (NeuWS) PDI technique was recently developed that combines high-resolution SLM based modulation with recent developments in machine learning (implicit neural representations~\cite{sitzmann2020implicit}) to image high-resolution, non-sparse static and dynamic scenes through severe optical aberrations~\cite{feng2023neuws}.
%NeuWS represents the state-of-the-art in guidestar-free imaging through scattering.

%Neural wavefront shaping is a breakthrough phase diversity imaging approach capable imaging through severe optical aberrations.


%Phase diversity imaging and NeuWS rely upon slow iterative algorithms and simple heuristics.


% Imaging through scattering is challenging because in general a scattering media's phase errors are unknown. 
% \textcolor{red}{Unknown and ill-posed are distinct problems. You could perfectly know the scattering media, but its forward model may not be invertible.}
% As a result, the inverse problems associated with imaging through scattering are often very ill-posed. 
% Imaging through scattering is challenging because the scattering process is lossy. 
% From the frequency domain perspective, the scattering media destroys some of the target scene's frequencies, either by destructively interfering with them or by scattering them outside the imaging sensor. If those frequencies are not captured in the measurement, it becomes difficult to faithfully recover them.

% %Imaging through scattering is hard
% Imaging through scattering is challenging because, in general, the scattering process is {\em unknown} and {\em lossy}. In the context of imaging an incoherent scene through an isoplanatic (spatially invariant) aberration, imaging through scattering can be framed as a blind deconvolution problem. In general, to image through scattering one must both recover the scattering-induced blur kernel and then invert (optically or computational) the scattering process to recover missing frequency content in the image.

%the noisy and corrupted measurements $I$ are related to the object of interest $O$ through 
% \begin{align}
%     I=O*H+Z,
% \end{align}
% where $H$ denotes an unknown blur kernel and $Z$ denotes denotes.




% %How existing methods deal with the imaging through scattering problem
% Many techniques have been developed to image through scattering media. If can can create a contre

% To recover the missing signal frequencies due to scattering media, most existing methods rely on prior information of the target scene, either hand-crafted or data-driven. Hand-crafted priors include but are not limited to total variation and Tikhonov regularization. Alternatively, data-driven priors require training a neural network to learn the mapping between distorted measurements and clean target scenes. A trained neural network can be either directly used to predict an estimate of the target in a feed-forward manner, or integrated into iterative optimization frameworks. 

% roughly fall into two categories: (1) data-driven supervised learning approaches and (2) unsupervised iterative optimization approaches. However, both categories suffer from said ill-posedness issue. As a result, data-driven feed-forward approaches tend to hallucinate realistic yet fake features in their reconstruction, while unsupervised approaches might lead to undesired artifacts, and tend to be much slower than feed-forward approaches.  Efforts have been made to fuse the two categories by using a data-driven neural network as a regularizer for iterative optimization approaches, 
 
% Although the aforementioned priors can help fill in the missing frequencies, they do not fundamentally escape the ill-posed nature of this problem --- they merely circumvent it by ``guessing'' or ``hallucinating'' the missing frequencies based on the preserved ones. The more frequencies are destroyed by the scattering media, the more inaccurate and error prone these reconstructions become. 
% Phase diversity imaging provides a mechanism to prevent these frequencies from being destroyed in the first place.
% %But can we prevent these frequencies from being destroyed in the first place? Yes, through phase diversity imaging. 

%\textcolor{red}{Need to rework this transition. PDI has been around for 30 years.}
%Recently, phase diversity imaging has emerged as a promising tool for imaging through scattering media, thanks to the development of deformable mirror arrays and spatial light modulators (SLM). These devices are able to arbitrarily shape the wavefront of incoming light by displaying phase modulation patterns in real-time (up to 1,000 fps). 
%\subsection{Phase Diversity Imaging}


%Phase diversity imaging, \textcolor{red}{illustrated in Figure XXX}, works by capturing a sequence of measurements -- each time the camera captures one measurement through the scattering media with a different phase modulation pattern. Its key idea is that a single phase modulation can make some of the frequencies better preserved, and make others worse preserved; but by applying multiple phase modulations in sequence, every frequency gets better preserved by at least one of the phase modulations; thus by leveraging all measurements, it can reduce ill-posedness. Recent works have demonstrated the advantage of phase diversity imaging via unsupervised iterative optimization approaches, of which the used phase modulation sequences are chosen by simple heuristics.



% Recent works have demonstrated the superior advantage of phase diversity imaging by using generic algorithms and neural representation, both of which are done in an unsupervised and iterative manner. 

% It should also be noted that this "multiple phase modulation" ability makes this line of work fundamentally different from the usage of single phase mask, as single phase mask would not be able to 


% It should be noted that this "multiple phase modulation" ability makes phase diversity imaging fundementally different from. 

% This differs from single phase mask that xxx.In comparison to using a single phase mask, 
% talk about single phase mask.

In this paper, we take a significant step towards a more systematic and principled approach in designing effective modulations that induces phase diversity during image acquisition. 
Moving beyond the traditional reliance on simple heuristics for determining modulation patterns, our method combines the strengths of differentiable optimization and data-driven learning.
Central to our approach is the novel integration of the optical model of wavefront modulations with a {\it proxy} reconstruction network, resulting in a fully differentiable system.
This integration allows for the simultaneous optimization of both the proxy reconstruction network and the modulation patterns, which are optimized end-to-end based on a large, simulated training dataset.
While imaging through scattering often requires iterative optimization algorithms because deep-learned feedforward networks often fail to generalize outside their training domain, this paper presents an intriguing twist by showing that, the training of a {\it hard-to-generalize} network can actually become a useful proxy for us to learn {\it generalizable} modulations.
Crucially, this proxy feedforward network allows us to bypass the expensive backpropagation computation through an iterative reconstruction algorithm, which would be necessary, but hopelessly impractical, if we were to naively optimize the modulations: each optimization step would require us to finish an entire iterative reconstruction algorithm.
As will be shown in our extensive experiments on both simulated and real-world captures, our learned modulations significantly enhance the reconstruction capability of both our deep-learned feedforward proxy network and a state-of-the-art iterative optimization-based method for imaging through scattering.
%Our framework is distinct in its ability to integrate data-driven insights about the scattering impact on wavefront into the design of wavefront modulations.
%Furthermore, the versatility of our framework is highlighted by its dual functionality: while our trained network exhibits strong generalization capabilities on unseen test data captured with our learned modulations, the modulations can also be effortlessly incorporated into existing imaging methods that employ iterative optimization.

%\subsection{Our Contribution}

% \textcolor{red}{I don't like this paragraph's narrative. This reads as improving how priors are incorporated. I'd prefer to talk about introducing a principled and powerful way to select modulation patterns.}

% To recover the missing signal frequencies due to scattering media, most existing methods rely on prior information of the target scene, either hand-crafted or data-driven. Hand-crafted priors include but are not limited to total variation and Tikhonov regularization. Alternatively, data-driven priors require training a neural network to learn the mapping between distorted measurements and clean target scenes. A trained neural network can be either directly used to predict an estimate of the target in a feed-forward manner, or integrated into iterative optimization frameworks. 

% With the knowledge of phase diversity imaging in mind, let us rethink the strategy of incorporating prior knowledge. While the research community has spent a ton of efforts on imposing priors in the image space to improve the image reconstruction quality,  we explore a new research direction: \textit{can we impose prior information on the design of phase-modulation-sequence such that the resulted phase diversity imaging system can preserve more frequencies?} It should be noted that the latter direction is complementary to the former -- if more frequencies get preserved, then subsequently, the problem would become much less ill-posed, and the priors on image space would also work better. 

%This paper develops a powerful learning-based approach for designing and optimizing PDI modulation patterns and reconstruction algorithms. 
%Our approach integrates differentiable optical models with feedforward image reconstruction algorithms to form a fully differentiable model of our imaging system that we can optimize end-to-end with training data and back-propagation. 

%optimize a learning-based PDI system end-to-end

%designing and optimizing learning-based phase diversity imaging systems.

%Contrary to the heuristically chosen phase modulation sequences used in previous phase diversity imaging approaches, in this work, we propose to use end-to-end learning to embed prior information of scattering media into our phase modulation sequence design. With a differentiable model for scattering media, our phase modulation sequence is jointly optimized with a feed-forward reconstruction neural network.  

The contributions of this paper include:
\begin{itemize}[leftmargin=.3in]
  \item We present a novel end-to-end learning framework to optimize wavefront modulations during acquisition to enhance our abilities to see through scattering.
  \item We demonstrate in both simulated and physical experiments that our learned modulations substantially improve image reconstruction quality and effectively generalize to unseen targets and scattering media.
  \item We show that the learned modulations can be decoupled from the jointly-trained proxy reconstruction network and significantly enhance the reconstruction quality of state-of-the-art unsupervised approaches.
  \end{itemize}

% We hope that our work can inspire the research community to to

% More specifically, we make the following contributions:. In this work, we investigate the optimal design of phase modulation sequence, in hope of preserving the most amount of frequency information against scattering media. 

% However, one limitation of previous wavefront modulation methods is that they use randomly generated modulation patterns. It has not yet been investigated whether using randomly generated phase modulation patterns leads to sub-optimal performance. In this paper, we make the following contributions:

% a new research direction. We hope that our work can inspire the research community to 

% ts key idea being improving the conditioning of the imaging system. More specifically, 
    

% \subsection{Contributions}




\fi



==> backup/1_intro_chris_no_comments.tex <==
\section{Introduction}
\label{sec:intro}
Scattering and related optical aberrations are ubiquitous in imaging and can be caused by a broad range of factors including fog, raindrops, murky water, atmospheric turbulence, fiber bundles, and human skin and tissue~\cite{gigan2022roadmap,yoon2020deep,watnik2018wavefront}. When light passes through such media, its phase is irregularly delayed and
its ``wavefront'' becomes distorted. These distortions blur and warp any images captured through
the scatterer. Solving the imaging-through-scattering problem would have profound implications in autonomous navigation, microscopy, endoscopy, astronomy, remote sensing, and other applications.

\begin{figure}[t]
  \centering
   \includegraphics[width=\linewidth]{sec/figs/teaser.pdf}
   \caption{\textbf{Learned Wavefront Modulations}. During image acquisition, we shape the wavefront of scattered light with a series of learned modulation patterns and capture a set of image measurements. 
   %We can then solve a maximum-likelihood estimation problem (or employ a feedforward neural network) to recover the obstructed scene. 
   We can then recover the scene behind the scattering medium by feeding the modulated measurements to supervised or unsupervised reconstruction methods.
   Using a state-of-the-art unsupervised method~\cite{feng2023neuws}, our learned modulations drastically improve the reconstruction quality compared to the previous approach~\cite{feng2023neuws} that applies random modulations during acquisition.}
   \label{fig:onecol}
\end{figure}

From the frequency domain perspective, the effect of an (incoherently illuminated) scene passing through scattering is the destruction/filtering of frequency content. 
Recovering these lost frequencies is very difficult using purely computational methods. %A question naturally arises: Can we modify the measurement process to prevent the loss of information during acquisition? 
Wavefront modulation and phase diversity imaging are powerful approaches to image through optical aberrations which modify the measurement process to preserve and recover frequency content.  
These methods captures a sequence of measurements where each measurement introduces an additional {known} wavefront error---typically just defocus---into the measurement~\cite{gonsalves1982phase,paxman1992joint,vogel1998fast,thelen1999maximum,kner2013phase,xin2019object,kang2023coordinate,reiser2023phase}. Much like the coded diffraction patterns employed in the context of phase retrieval~\cite{candes2015phaseCDP}, this modulation process adds diversity to the measurements and makes the obstructed scene easier to reconstruct. 

Until recently, such approaches were restricted to imaging simple scenes through the relatively mild (smooth and regular) optical aberrations.
However, a breakthrough neural wavefront shaping (NeuWS) technique was recently developed that combines high-resolution SLM based modulation with recent developments in machine learning (implicit neural representations~\cite{sitzmann2020implicit}) to image high-resolution, non-sparse static and dynamic scenes through severe optical aberrations~\cite{feng2023neuws}.
NeuWS represents the state-of-the-art in guidestar-free imaging through scattering.

\subsection{Our Contribution}

This paper develops a powerful learning-based approach for designing and optimizing wavefront modulation patterns. 
Our approach integrates differentiable optical models with feedforward {\em proxy} image reconstruction algorithms to form a fully differentiable model of our imaging system that we can optimize end-to-end with training data and back-propagation. 

While imaging through scattering often requires iterative optimization algorithms because deep-learned feedforward networks often fail to generalize outside their training domain, this paper demonstrates the remarkable finding that training a {\it hard-to-generalize} network can become a useful proxy allowing us to learn {\it generalizable} modulations.
Crucially, this proxy feedforward network allows us to bypass the expensive backpropagation computation through an iterative reconstruction algorithm, which would be necessary, but hopelessly impractical, if we were to naively optimize the modulations: each optimization step would require us to finish an entire iterative reconstruction algorithm.
As will be shown in our extensive experiments on both simulated and real-world data, our learned modulations significantly enhance the reconstruction capability of both our deep-learned feedforward proxy network and a state-of-the-art iterative optimization-based method for imaging through scattering.

The contributions of this paper include:
\begin{itemize}[leftmargin=.3in]
  \item We present a novel end-to-end learning framework to optimize wavefront modulations during acquisition to enhance our abilities to see through scattering.
  \item We demonstrate in both simulated and physical experiments that our learned modulations substantially improve image reconstruction quality and effectively generalize to unseen targets and scattering media.
  \item We show that the learned modulations can be decoupled from the jointly-trained proxy reconstruction network and significantly enhance the reconstruction quality of state-of-the-art unsupervised approaches.
  \end{itemize}

